DIALOG-22 RuATD Generated Text Detection

Text Generation Models (TGMs) succeed in creating text that matches human language style reasonably well. Detectors that can distinguish between TGM-generated text and human-written ones play an important role in preventing abuse of TGM. In this paper, we describe our pipeline for the two DIALOG-22 RuATD tasks: detecting generated text (binary task) and classification of which model was used to generate text (multiclass task). We achieved 1st place on the binary classification task with an accuracy score of 0.82995 on the private test set and 4th place on the multiclass classification task with an accuracy score of 0.62856 on the private test set. We proposed an ensemble method of different pre-trained models based on the attention mechanism.

==> dialogue <==
\begin{thebibliography}{}

\bibitem[\protect\citename{Antuhov}2020]{habr_2020}
Denis Antuhov.
\newblock 2020.
\newblock Natulral language model learning with bert and tensorflow
  link:https://habr.com/ru/company/sberdevices/blog/527576/, Nov.

\bibitem[\protect\citename{Conneau \bgroup et al.\egroup
  }2018]{conneau2018xnli}
Alexis Conneau, Guillaume Lample, Ruty Rinott, Adina Williams, Samuel~R Bowman,
  Holger Schwenk, and Veselin Stoyanov.
\newblock 2018.
\newblock Xnli: Evaluating cross-lingual sentence representations.
\newblock {\em arXiv preprint arXiv:1809.05053}.

\bibitem[\protect\citename{Conneau \bgroup et al.\egroup
  }2019]{conneau2019unsupervised}
Alexis Conneau, Kartikay Khandelwal, Naman Goyal, Vishrav Chaudhary, Guillaume
  Wenzek, Francisco Guzm{\'a}n, Edouard Grave, Myle Ott, Luke Zettlemoyer, and
  Veselin Stoyanov.
\newblock 2019.
\newblock Unsupervised cross-lingual representation learning at scale.
\newblock {\em arXiv preprint arXiv:1911.02116}.

\bibitem[\protect\citename{Devlin \bgroup et al.\egroup }2018]{devlin2018bert}
Jacob Devlin, Ming-Wei Chang, Kenton Lee, and Kristina Toutanova.
\newblock 2018.
\newblock Bert: Pre-training of deep bidirectional transformers for language
  understanding.
\newblock {\em arXiv preprint arXiv:1810.04805}.

\bibitem[\protect\citename{Dugan \bgroup et al.\egroup }2020]{dugan2020roft}
Liam Dugan, Daphne Ippolito, Arun Kirubarajan, and Chris Callison-Burch.
\newblock 2020.
\newblock Roft: A tool for evaluating human detection of machine-generated
  text.
\newblock {\em arXiv preprint arXiv:2010.03070}.

\bibitem[\protect\citename{Gehrmann \bgroup et al.\egroup
  }2019]{gehrmann2019gltr}
Sebastian Gehrmann, Hendrik Strobelt, and Alexander~M Rush.
\newblock 2019.
\newblock Gltr: Statistical detection and visualization of generated text.
\newblock {\em arXiv preprint arXiv:1906.04043}.

\bibitem[\protect\citename{Gusev}2020]{gusev2020dataset}
Ilya Gusev.
\newblock 2020.
\newblock Dataset for automatic summarization of russian news.
\newblock  // {\em Conference on Artificial Intelligence and Natural Language},
  P 122--134. Springer.

\bibitem[\protect\citename{He \bgroup et al.\egroup }2021]{he2021debertav3}
Pengcheng He, Jianfeng Gao, and Weizhu Chen.
\newblock 2021.
\newblock Debertav3: Improving deberta using electra-style pre-training with
  gradient-disentangled embedding sharing.
\newblock {\em arXiv preprint arXiv:2111.09543}.

\bibitem[\protect\citename{Ippolito \bgroup et al.\egroup
  }2019]{ippolito2019automatic}
Daphne Ippolito, Daniel Duckworth, Chris Callison-Burch, and Douglas Eck.
\newblock 2019.
\newblock Automatic detection of generated text is easiest when humans are
  fooled.
\newblock {\em arXiv preprint arXiv:1911.00650}.

\bibitem[\protect\citename{Jawahar \bgroup et al.\egroup
  }2020]{jawahar2020automatic}
Ganesh Jawahar, Muhammad Abdul-Mageed, and Laks~VS Lakshmanan.
\newblock 2020.
\newblock Automatic detection of machine generated text: A critical survey.
\newblock {\em arXiv preprint arXiv:2011.01314}.

\bibitem[\protect\citename{Liu \bgroup et al.\egroup
  }2020]{liu2020multilingual}
Yinhan Liu, Jiatao Gu, Naman Goyal, Xian Li, Sergey Edunov, Marjan
  Ghazvininejad, Mike Lewis, and Luke Zettlemoyer.
\newblock 2020.
\newblock Multilingual denoising pre-training for neural machine translation.
\newblock {\em Transactions of the Association for Computational Linguistics},
  8:726--742.

\bibitem[\protect\citename{Sber}2022]{sberbank-ai}
Sber.
\newblock 2022.
\newblock Sberbank-ai.
\newblock \url{https://huggingface.co/sberbank-ai}.

\bibitem[\protect\citename{Shamardina \bgroup et al.\egroup
  }2022a]{shamardina2022ruatd}
Tatiana Shamardina, Vladislav Mikhailov, Daniil Chernianskii, Alena Fenogenova,
  Marat Saidov, Anastasiya Valeeva, Tatiana Shavrina, Ivan Smurov, Elena
  Tutubalina, and Ekaterina Artemova.
\newblock 2022a.
\newblock {Findings of the The RuATD Shared Task 2022 on Artificial Text
  Detection in Russian}.
\newblock  // {\em Computational Linguistics and Intellectual Technologies:
  Papers from the Annual Conference "Dialogue"}, volume~21, P xxx--xxx.

\bibitem[\protect\citename{Shamardina \bgroup et al.\egroup
  }2022b]{ruatd-2022-binary}
Tatiana Shamardina, Vladislav Mikhailov, Daniil Chernianskii, Alena Fenogenova,
  Marat Saidov, Anastasiya Valeeva, Tatiana Shavrina, Ivan Smurov, Elena
  Tutubalina, and Ekaterina Artemova.
\newblock 2022b.
\newblock Ruatd 2022 (binary task).
\newblock \url{https://www.kaggle.com/competitions/ruatd-2022-bi}.
\newblock Accessed: 2022-03-28.

\bibitem[\protect\citename{Shamardina \bgroup et al.\egroup
  }2022c]{ruatd-2022-multiclass}
Tatiana Shamardina, Vladislav Mikhailov, Daniil Chernianskii, Alena Fenogenova,
  Marat Saidov, Anastasiya Valeeva, Tatiana Shavrina, Ivan Smurov, Elena
  Tutubalina, and Ekaterina Artemova.
\newblock 2022c.
\newblock Ruatd 2022 (multi task).
\newblock \url{https://www.kaggle.com/competitions/ruatd-2022-multi-task}.
\newblock Accessed: 2022-03-28.

\bibitem[\protect\citename{Solaiman \bgroup et al.\egroup
  }2019]{solaiman2019release}
Irene Solaiman, Miles Brundage, Jack Clark, Amanda Askell, Ariel Herbert-Voss,
  Jeff Wu, Alec Radford, Gretchen Krueger, Jong~Wook Kim, Sarah Kreps, et~al.
\newblock 2019.
\newblock Release strategies and the social impacts of language models.
\newblock {\em arXiv preprint arXiv:1908.09203}.

\bibitem[\protect\citename{Wenzek \bgroup et al.\egroup
  }2020]{wenzek-etal-2020-ccnet}
Guillaume Wenzek, Marie-Anne Lachaux, Alexis Conneau, Vishrav Chaudhary,
  Francisco Guzm{\'a}n, Armand Joulin, and Edouard Grave.
\newblock 2020.
\newblock {CCN}et: Extracting high quality monolingual datasets from web crawl
  data.
\newblock  // {\em Proceedings of the 12th Language Resources and Evaluation
  Conference}, P 4003--4012, Marseille, France, May. European Language
  Resources Association.

\bibitem[\protect\citename{Williams \bgroup et al.\egroup
  }2017]{williams2017broad}
Adina Williams, Nikita Nangia, and Samuel~R Bowman.
\newblock 2017.
\newblock A broad-coverage challenge corpus for sentence understanding through
  inference.
\newblock {\em arXiv preprint arXiv:1704.05426}.

\bibitem[\protect\citename{Wolf \bgroup et al.\egroup
  }2020]{wolf2020transformers}
Thomas Wolf, Lysandre Debut, Victor Sanh, Julien Chaumond, Clement Delangue,
  Anthony Moi, Pierric Cistac, Tim Rault, R{\'e}mi Louf, Morgan Funtowicz,
  et~al.
\newblock 2020.
\newblock Transformers: State-of-the-art natural language processing.
\newblock  // {\em Proceedings of the 2020 conference on empirical methods in
  natural language processing: system demonstrations}, P 38--45.

\end{thebibliography}

